Taylor Moment Expansion for Continuous-Discrete Gaussian Filtering and Smoothing

The paper is concerned with non-linear Gaussian filtering and smoothing in continuous-discrete state-space models, where the dynamic model is formulated as an It\^{o} stochastic differential equation (SDE), and the measurements are obtained at discrete time instants. We propose novel Taylor moment expansion (TME) Gaussian filter and smoother which approximate the moments of the SDE with a temporal Taylor expansion. Differently from classical linearisation or It\^{o}--Taylor approaches, the Taylor expansion is formed for the moment functions directly and in time variable, not by using a Taylor expansion on the non-linear functions in the model. We analyse the theoretical properties, including the positive definiteness of the covariance estimate and stability of the TME Gaussian filter and smoother. By numerical experiments, we demonstrate that the proposed TME Gaussian filter and smoother significantly outperform the state-of-the-art methods in terms of estimation accuracy and numerical stability.

==> figs/banner.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%Straight Lines [id:da4950933627624654] 
\draw [color={rgb, 255:red, 119; green, 172; blue, 48 }  ,draw opacity=1 ][line width=1.5]    (394,73) -- (517,72.02) ;
\draw [shift={(520,72)}, rotate = 539.55] [color={rgb, 255:red, 119; green, 172; blue, 48 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da44070739825699423] 
\draw [line width=1.5]    (223,122) -- (350.08,151.33) ;
\draw [shift={(353,152)}, rotate = 192.99] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da5963580976637393] 
\draw [color={rgb, 255:red, 0; green, 114; blue, 189 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (440,152) -- (517,152) ;
\draw [shift={(520,152)}, rotate = 180] [color={rgb, 255:red, 0; green, 114; blue, 189 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da6419588129795044] 
\draw [color={rgb, 255:red, 237; green, 177; blue, 32 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (410,222) -- (517.05,202.54) ;
\draw [shift={(520,202)}, rotate = 529.7] [color={rgb, 255:red, 237; green, 177; blue, 32 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da5531182354276991] 
\draw [line width=1.5]    (390,172) -- (390,219) ;
\draw [shift={(390,222)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da534581519886506] 
\draw [color={rgb, 255:red, 217; green, 83; blue, 25 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (410,242) -- (517.05,261.46) ;
\draw [shift={(520,262)}, rotate = 190.3] [color={rgb, 255:red, 217; green, 83; blue, 25 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da7379917111079921] 
\draw [color={rgb, 255:red, 119; green, 172; blue, 48 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (223,92) -- (350.03,72.46) ;
\draw [shift={(353,72)}, rotate = 531.25] [color={rgb, 255:red, 119; green, 172; blue, 48 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da6942446487652874] 
\draw [line width=1.5]    (640,152) -- (687,152) ;
\draw [shift={(690,152)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Rounded Rect [id:dp9638124790744704] 
\draw  [dash pattern={on 5.63pt off 4.5pt}][line width=1.5]  (540,58) .. controls (540,49.16) and (547.16,42) .. (556,42) -- (604,42) .. controls (612.84,42) and (620,49.16) .. (620,58) -- (620,276) .. controls (620,284.84) and (612.84,292) .. (604,292) -- (556,292) .. controls (547.16,292) and (540,284.84) .. (540,276) -- cycle ;
%Straight Lines [id:da6629782569030249] 
\draw [color={rgb, 255:red, 119; green, 172; blue, 48 }  ,draw opacity=1 ][line width=1.5]    (20,200) -- (60,200) ;


%Straight Lines [id:da7067908163607981] 
\draw [color={rgb, 255:red, 0; green, 114; blue, 189 }  ,draw opacity=1 ]   (20,220) -- (60,220) ;


%Straight Lines [id:da9181552410040403] 
\draw [color={rgb, 255:red, 237; green, 177; blue, 32 }  ,draw opacity=1 ][fill={rgb, 255:red, 217; green, 83; blue, 25 }  ,fill opacity=1 ][line width=1.5]    (20,240) -- (60,240) ;


%Straight Lines [id:da8959649782846455] 
\draw [color={rgb, 255:red, 217; green, 83; blue, 25 }  ,draw opacity=1 ][line width=1.5]    (20,260) -- (60,260) ;


%Straight Lines [id:da9491478418054853] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (20,280) -- (57,280) ;
\draw [shift={(60,280)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da19144142698708855] 
\draw [line width=1.5]    (20,300) -- (57,300) ;
\draw [shift={(60,300)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Shape: Rectangle [id:dp3330663643244942] 
\draw  [dash pattern={on 5.63pt off 4.5pt}][line width=1.5]  (10,180) -- (230,180) -- (230,320) -- (10,320) -- cycle ;


% Text Node
\draw (375,71) node   {$\hat{\mathbf{x}}(t)$};
% Text Node
\draw (579,76) node   {$\mathbb{E}\left[ \phi\left(\hat{\mathbf{x}}(t)\right)\right]$};
% Text Node
\draw (119,82) node  [align=left] {SDE};
% Text Node
\draw (120,108) node   {$\mathrm{d}\mathbf{x} \ =\ \mathbf{f}(\mathbf{x}, t) \ \mathrm{d} t\ +\ \mathbf{L}(\mathbf{x}, t) \ \mathrm{d}\mathbf{W}_{t}$};
% Text Node
\draw (281.46,67.71) node [rotate=-351.11] [align=left] {Discretise};
% Text Node
\draw (451.5,61) node  [align=left] {Moment functions};
% Text Node
\draw (395,151) node   {$\mathbb{E}[ \phi(\mathbf{x}(t))]$};
% Text Node
\draw (277.35,148.88) node [rotate=-13.64] [align=left] { It\^{o}'s lemma};
% Text Node
\draw (577,153) node   {$\hat{\mathbb{E}}[ \phi (\mathbf{x}(t))]$};
% Text Node
\draw (577,203) node   {$\hat{\mathbb{E}}[ \phi (\mathbf{x}(t))]$};
% Text Node
\draw (475.5,141) node  [align=left] {Discretise};
% Text Node
\draw (390.5,233) node  [align=left] {ODEs};
% Text Node
\draw (577,267) node   {$\hat{\mathbb{E}}[ \phi (\mathbf{x}(t))]$};
% Text Node
\draw (458.7,200.03) node [rotate=-349.25] [align=left] {Linearise};
% Text Node
\draw (456.12,271.13) node [rotate=-11.59] [align=center] {Gaussian\\assumption};
% Text Node
\draw (754.5,149) node  [align=center] {Gaussian filtering\\and\\smoothing};
% Text Node
\draw (484.5,232) node  [align=left] {ODEs solver};
% Text Node
\draw (97.5,200) node [scale=0.7] [align=left] {It\^{o}-Taylor};
% Text Node
\draw (145,219) node [scale=0.7] [align=left] {Taylor moment expansion (TME)};
% Text Node
\draw (104,240) node [scale=0.7] [align=left] {Linear-ODEs};
% Text Node
\draw (103,259) node [scale=0.7] [align=left] {Gauss-ODEs};
% Text Node
\draw (121,280) node [scale=0.7] [align=left] {Estimatied derivation};
% Text Node
\draw (115,299) node [scale=0.7] [align=left] {Explicit derivation};
\end{tikzpicture}


==> figs/differences.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300


%Straight Lines [id:da30240109029295614] 
\draw [line width=1.5]    (160,60) -- (247,60) ;
\draw [shift={(250,60)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

%Straight Lines [id:da43614197888351525] 
\draw [line width=1.5]    (160,100) -- (247,100) ;
\draw [shift={(250,100)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

%Straight Lines [id:da30378801160595836] 
\draw [line width=1.5]    (160,140) -- (247,140) ;
\draw [shift={(250,140)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

%Straight Lines [id:da24400885139806872] 
\draw [line width=1.5]    (180,40) -- (180,56.65) ;
\draw [shift={(180,60)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]      (0, 0) circle [x radius= 3.36, y radius= 3.36]   ;

%Straight Lines [id:da5381976029341229] 
\draw [line width=1.5]    (200,40) -- (200,96.65) ;
\draw [shift={(200,100)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]      (0, 0) circle [x radius= 3.36, y radius= 3.36]   ;

%Straight Lines [id:da2282295847092517] 
\draw [line width=1.5]    (220,40) -- (220,136.65) ;
\draw [shift={(220,140)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]      (0, 0) circle [x radius= 3.36, y radius= 3.36]   ;


% Text Node
\draw (113.5,61) node  [align=left] {EKF};
% Text Node
\draw (115.5,101) node  [align=left] {It\^{o}--Taylor};
% Text Node
\draw (112,141) node  [align=left] {TME};
% Text Node
\draw (321,97) node   {$\phi \left(\mathbf{x}_{t}\right)$};
% Text Node
\draw (320.5,140) node   {$\expec[\phi(\cu{x})]$};
% Text Node
\draw (284.5,60.5) node   {$\cu{f}(\mathbf{x}_{t},  t)$};
% Text Node
\draw (325.5,61) node  [align=left] {and};
% Text Node
\draw (372.5,60.5) node   {$\cu{L}( \cu{x}_{t},  t)$};
% Text Node
\draw (201.5,31) node  [align=left] {Taylor expansion};


\end{tikzpicture}

